Go Wide, Then Narrow: Efficient Training of Deep Thin Networks

For deploying a deep learning model into production, it needs to be both accurate and compact to meet the latency and memory constraints. This usually results in a network that is deep (to ensure performance) and yet thin (to improve computational efficiency). In this paper, we propose an efficient method to train a deep thin network with a theoretic guarantee. Our method is motivated by model compression. It consists of three stages. First, we sufficiently widen the deep thin network and train it until convergence. Then, we use this well-trained deep wide network to warm up (or initialize) the original deep thin network. This is achieved by layerwise imitation, that is, forcing the thin network to mimic the intermediate outputs of the wide network from layer to layer. Finally, we further fine tune this already well-initialized deep thin network. The theoretical guarantee is established by using the neural mean field analysis. It demonstrates the advantage of our layerwise imitation approach over backpropagation. We also conduct large-scale empirical experiments to validate the proposed method. By training with our method, ResNet50 can outperform ResNet101, and BERT Base can be comparable with BERT Large, when ResNet101 and BERT Large are trained under the standard training procedures as in the literature.

==> old_derivation.tex <==
%\iffal
\section{Derivation}
\\
\textcolor{red}{[Unify notation later]}
Assume $F^*$ is the true model. Let $N$ be the width of the wide network $\hat F$ (assume all the layers have equal width for now), and $n$ the width of the narrow network. Let $d$ be the depth of both $\hat F$ and $\hat f$. 

We plan to prove the following theorem. 
\begin{theorem}
%\begin{e}
%1. Directly training
If we take $\widehat{F}$ sufficiently wide such that $N = O(d^2\exp(2d)/{n}) $, we have %obtain %the final result:
$$
 \norm{\hat f -  F^*}_{\mathcal D}  
  = O\left (\frac{d}{\sqrt{n}}\right). 
$$
Note that the error scales linearly with the depth $d$. 
In contrast, if we directly train a narrow network of width $n$ starting from scratch using SGD, we would get  $\norm{\hat f -  F^*}_{\mathcal D}   = O\left (\frac{\exp(d)}{\sqrt{n}}\right)$.
\end{theorem}

\paragraph{Proof Outline}
\begin{enumerate}
\item Show that the wider network achieves a $O(\exp(d)/\sqrt{N})$ error, that is, 
$$
\norm{\widehat{F} - F^*}_{\mathcal D} = O\left (\frac{\exp(d)}{\sqrt{N}}\right). 
$$
In addition, we need to show that $\hat F$ is sufficiently Lipschitz in that 
\begin{align}\label{equ:jj}
\prod_{j=\ell+1}^d\norm{\hat F_j}_{Lip} \leq %\norm{F^*}_{Lip} 
L^*+ O\left (\frac{\exp(d)}{\sqrt{N}}\right), ~~~~~\forall \ell = 1,\ldots, d-1,  
\end{align}
for some constant $L^*$ that depends on the Lipschitz of the true function $F^*$.  \textcolor{red}{This is key difficulty.}
\item Show that $\epsilon_1 := \norm{\hat f_1 - \hat F_1}_{\mathcal D}  = O(1/\sqrt{n})$. More generally, show that 
$$
\epsilon_\ell := \norm{\hat f_\ell - \hat F_\ell}_{\mathcal D_{\ell-1}} 
:= \norm{\hat f_\ell \circ \hat f_{\ell-1:1} -\hat  F_\ell \circ \hat f_{\ell-1:1}}_{\mathcal D}  = O(1/\sqrt{n}), 
$$ 
where $\mathcal D_{\ell-1}$ denotes the distribution we obtained by applying $\hat f_{\ell-1:1}$ on the original data  $\mathcal D$. 
\item Show that 
\begin{align*} 
E_2:= \norm{\hat f_2 \circ \hat f_1 -\hat  F_2 \circ \hat F_1}_{\mathcal D}
& \leq 
\norm{\hat f_2 \circ \hat f_1 -\hat  F_2 \circ \hat f_1}_{\mathcal D}  + \norm{\hat F_2 \circ \hat f_1 -\hat  F_2 \circ \hat F_1}_{\mathcal D}  \\
& \leq \norm{\hat f_2 \circ \hat f_1 -\hat  F_2 \circ \hat f_1}_{\mathcal D}  ~+~  \norm{\hat F_2}_{Lip} \norm{\hat f_1  - \hat F_1}_{\mathcal D}  \\
& \leq \epsilon_2 +  \epsilon_1 \norm{\hat F_2}_{Lip}. 
\end{align*}
\item In general 
\begin{align*} 
E_\ell := \norm{\hat f_\ell \circ \hat f_{\ell-1:1} -\hat  F_\ell \circ \hat F_{\ell-1:1}}_{\mathcal D} 
& \leq 
\norm{\hat f_\ell \circ \hat f_{\ell-1:1} -\hat  F_\ell \circ \hat f_{\ell-1:1}}_{\mathcal D}  + \norm{\hat F_{\ell} \circ \hat f_{\ell-1:1} -\hat  F_\ell \circ \hat F_{\ell-1}}_{\mathcal D}  \\
& \leq \epsilon_\ell + \norm{\hat F_\ell}_{Lip} E_{\ell-1} 
%& \leq \norm{\hat f_2 \circ \hat f_1 -\hat  F_2 \circ \hat f_1} ~+~  \norm{\hat F_2}_{Lip} \norm{\hat f_1  - \hat F_1} \\
%& \leq \epsilon_\ell + \epsilon_ \norm{\hat F_2}_{Lip}. 
\end{align*}
%We have 
By recursion, we have 
$$E_3= \epsilon_3  +\norm{\hat F_3}_{Lip} \epsilon_2 +  \norm{\hat F_3}_{Lip}  \norm{\hat F_2}_{Lip} \epsilon_1 
$$
And in general, 
$$
E_d = \sum_{\ell=1}^d
\prod_{j=\ell+1}^d \norm{\hat F_j}_{Lip}   \epsilon_\ell.
$$
Following \eqref{equ:jj} and that $\epsilon_\ell = O(1/\sqrt{n})$, we obtain 
$$
 \norm{\hat f -  F^*}_{\mathcal D}  \leq 
  \norm{\hat f - \hat F}_{\mathcal D}   +  \norm{\hat F- F^*}_{\mathcal D}  
\norm{\hat f - \hat F}_{\mathcal D} = O\left (\left (L^*+ O\left (\frac{\exp(d)}{\sqrt{N}}\right)\right) \times \frac{d}{\sqrt{n}}\right ) + O\left (\frac{\exp(d)}{\sqrt{N}}\right).
$$
Therefore, if we take $N = O(d^2\exp(2d)/{n}) $, we obtain the final result:
$$
 \norm{\hat f - F^*}_{\mathcal D}  = O\left (\frac{d}{\sqrt{n}}\right). 
$$


\end{enumerate}

